Towards Confidence-aware Calibrated Recommendation

Recommender systems utilize users' historical data to learn and predict their future interests, providing them with suggestions tailored to their tastes. Calibration ensures that the distribution of recommended item categories is consistent with the user's historical data. Mitigating miscalibration brings various benefits to a recommender system. For example, it becomes less likely that a system overlooks categories with less interaction on a user's profile by only recommending popular categories. Despite the notable success, calibration methods have several drawbacks, such as limiting the diversity of the recommended items and not considering the calibration confidence. This work, presents a set of properties that address various aspects of a desired calibrated recommender system. Considering these properties, we propose a confidence-aware optimization-based re-ranking algorithm to find the balance between calibration, relevance, and item diversity, while simultaneously accounting for calibration confidence based on user profile size. Our model outperforms state-of-the-art methods in terms of various accuracy and beyond-accuracy metrics for different user groups.

==> bc/calibration_bc.tex <==
% \section{Motivating Calibration Limitations}
\section{Calibrated Recommendation}
\label{sec:method}

\subsection{Problem Definition}
\label{sec:problem_definition}
Let $\mathcal{U}$ and $\mathcal{I}$ be the set of consumers and items with sizes $n$ and $m$, respectively. Further, assume that there exists a set of categories $\mathcal{C}$ describing items in $\mathcal{I}$.  Categories can be either defined by the system designer, such as popular and unpopular items~\cite{abdollahpouri2020connection}, or intrinsic features of items, such as a movie genre (e.g., Action, Comedy).  In a typical recommender system, a user, $u \in \mathcal{U}$, is provided a list of top-N items, $L_N(u)$ according to a defined relevance score, $s \in S^{n\times N}$. To measure the degree of calibration of the recommendation list, following~\citet{steck2018calibrated}, we determine two distributions for the categories $c \in \mathcal{C}$; $p(c|u)$, for the rated items in a user profile, and $q(c|u)$ for the items in her recommendation list $L_N(u)$,. These distributions are formally defined as:

% the first distribution is for items rated by the user in the training set, $p(c|u)$, and the other is for items recommended to the user in $L_N(u)$, $q(c|u)$. These distributions are formally defined as:

\begin{small}
\begin{equation}
\label{eq:p}
p(c|u) = \frac{\sum_{i \in \mathcal{I}_u} w_{ui} \times \mathds{1}(c \in i) }{|\mathcal{I}_u| \times \sum_{i \in \mathcal{I}_u} w_{ui}}
\end{equation}
\begin{equation}
\label{eq:q}
q(c|u) = \frac{\sum_{i \in L_N(u)} w_{r(i)} \times \mathds{1}(c \in i) }{|L_N(u)| \times \sum_{i \in L_N(u)} w_{r(i)}}
\end{equation}
\end{small}

\noindent
where $\mathds{1}(c \in i)$ is an indicator function returning 1 when item $i$ has category $c$ and 0 otherwise. $\mathcal{I}_u$ is the set of items in the profile of user $u$. $w_{r(i)}$ is the weight of item $i$ given its rank, $r(i)$,  in the recommendation list (\eg logarithmic reduction factor based on rank similar to nDCG's weighting scheme~\cite{wang2013theoretical}) whereas $w_{ui}$ represents the weight of item $i$ for user $u$ (\eg based on how recently the item has been rated). Finally, similar to~\cite{steck2018calibrated}, the degree of miscalibration is calculated by directly computing the statistical distance between two distributions of $p(g|u)$ and $q(g|u)$. In this work, we adopt Hellinger distance defined as \(H(p,q) = \frac{|| \sqrt{p} - \sqrt{q}||_{2}}{\sqrt{2}}\) as well as Jensen-Shannon (JS) divergence to calculate a symmetric normalized score using KL divergence. The smaller values of JS and H indicate better performance in calibration where the perfect calibration occurs when they are equal to zero. The overall miscalibration metric, $\mathbf{MC}$, is calculated by averaging divergence values (\eg using JS or H functions) across all users.

% Among statistical distances that quantify the distance between two probability distributions, Kullback-Leibler (KL) divergence and Hellinger (H) are most commonly used in the literature~\cite{steck2018calibrated,abdollahpouri2020connection,seymen2021constrained}. 

% JS divergence is more useful in calibration application than KL divergence as it is well-defined when $q(c|u)=0$ or $p(c|u)=0$ with scores between 0 (identical) and 1 (maximally different). Thus, the divergence of $p$ from $q$ is the same as that of $q$ from $p$, or stated formally as $JS(p, q) = JS(q, p) =  \frac{1}{2} * KL(p, M) + \frac{1}{2} * KL(q, M)$ and $M= \frac{1}{2} * (p + q)$. 

% JS divergence has the advantage of being very sensitive to minor discrepancies in $p(c|u)$ and $q(c|u)$ while favoring more uniform distributions. 


\subsection{Desired Properties of Calibration}
\label{sec:property}

\begin{figure}
    \centering
    \subfloat[Beta PDF]
    {
        {
            \includegraphics[width=0.4\columnwidth]{figs/dist.pdf}
            \label{fig:beta_dist}%
        }
    }
    \subfloat[Miscalibration in Test vs.~Train]
    {
        {
            \includegraphics[width=0.4\columnwidth]{figs/testvstrain.pdf}
            \label{fig:testvstrain_diff_ml_100K}
        }
    }
    \caption{Calibration for users with different profile size}%
    \label{fig:motivation}%
\end{figure}

Here we present the desired properties of calibrated recommendations and explain how they affect the final recommendation before moving into our proposed model addressing them.

\partitle{P1: Relevance Property.}
Calibrated recommendations intend to reflect different interests of users, as indicated by their interaction history, with the same proportion in the recommended list. A greedy algorithm is often proposed to re-rank a baseline recommendation list. The first desired property is that calibrating categories should occur without sacrificing overall relevance to users. \citet{seymen2021constrained} illustrate that greedy calibrated algorithms such as \cite{steck2018calibrated, oh2011novel} fail to meet this essential requirement that leads to suboptimal recommendations.

\partitle{P2: Diversity Aspects.}
According to the literature, diversity is defined as minimal redundancy or similarity in the recommendation lists. Many studies such as \cite{bhaskara2016linear,zhang2008avoiding,hurley2011novelty} propose different ways to generate diverse recommendations. Some focus on achieving personalized diversity, i.e., recommendations should increase the ``good'' diversity for users, which is a more user-centric goal~\cite{dang2012diversity,teo2016adaptive,vargas2014coverage,Eskandanian2017PersonalizedDiv,Sonb2020Opp}. The goal of calibrated recommendations, however, is pure user-centric and improvements in diversity is a side-effect. In other words, it intends to recommend all item categories in which a user has shown any interests and in a way we also increase diversity. Although we increase catalog coverage slightly, users are not exposed to all the categories and, therefore might still get stuck in a filter bubble~\cite{pariser2011filter}. We intend to prevent shrinkage in the overall catalog coverage in our method.


% and does not consider diversity as a separate objective that might lead to a so-called "filter bubble".Imagine a user who has rated 70\% Comedy and 30\% romance movies in a world with three genres. Such users would receive the target distribution of 70\%:30\%:0\% of the same genres in the recommended list depriving them of the opportunity to interact with the third genre. 
% The second desired property in calibrated recommendation is to prevent such phenomenon by preventing a reduction in overall catalog coverage and diversity in comparison to baselines.  

\partitle{P3: Calibration Confidence.}
Calibrated recommendations are solely based on users' historical interactions. As discussed earlier, the profile of users influence the level of confidence an algorithm has while calibrating the user profile. This can also be seen from a temporal perspective where users tend to change their taste over time. Therefore, the less we know about a user's past interactions (i.e., smaller profile size), the less we can be sure of their future taste and its change. To investigate this issue, along with the theoretical analysis of Beta distributions (see Section~\ref{sec:intro}), we perform a temporal split of the data into train/test scenarios. For this example, we consider the test data as an oracle recommendation algorithm that can make perfect predictions, \ie return the ground truth. Figure~\ref{fig:testvstrain_diff_ml_100K} depicts the degree of miscalibration for the oracle algorithm as defined in Section~\ref{sec:problem_definition}. To analyze the miscalibration effect from the user's perspective, we categorize the users into three groups based on their activity level, \ie number of interactions. The top 20$\%$ of users are categorized as \uga~group while the bottom 20$\%$ are assigned \ugc~group, and the remainder is categorized as \ugb~group. As we can see from the values of JS and H in Figure~\ref{fig:testvstrain_diff_ml_100K}, the accuracy-optimal oracle algorithm fails to calibrate the recommendation list according to genres distribution, especially for the \ugc~group followed by the \ugb~group. This result indicates that modeling user preference towards genre is more challenging for less active users, and considerable training data is needed to capture the user's taste in categories with high confidence. This is also evident in Figure~\ref{fig:beta_dist} where we see a ~0.67 higher confidence when modeling the user with a larger profile size. Hence, calibrating recommendations for all users to the same degree regardless of their profile length leads to undesired recommendations motivating the need for calibrated recommendations without limiting baseline recommendation algorithms' predictive ability for less active users. State-of-the-art recommendation models are designed to make predictions of users' dynamic behavior. Hence, the third desired property in calibration is to have a varying degree of calibration for less active users while benefiting from the baseline algorithm's predictive ability. 

\subsection{Proposed Model}
In the following, we describe our proposed confidence-aware calibrated algorithm that meet the desired properties mentioned in Section~\ref{sec:property}. The purpose of the algorithm is to re-rank a baseline recommendation ranking list, $L_N(u)$, in a way that the new top-K list, $L_K^c(u)$ where $K<N$, would reduce miscalibration without limiting baseline algorithm predictive ability. To this end, we define binary matrix $Z=[Z_{ui}]_{n \times N}$ to denote whether item $i \in \mathcal{I}$ is recommended to user $u \in \mathcal{U}$ in $L_K^c(u)$. Hence, we can represent $L_K^c(u)$ as $[Z_{u1}, Z_{u2}, ..., Z_{uN}]$ when $\sum_{i=1}^{N}{Z_{ui}} = K$. Let $W(I_u) \in [0,1]$ denote the confidence weight given user $u$ based on the rated items in her profile, $I_u$. The confidence weight aims to represent the degree of calibration for user u where 1 indicate that the model would fully calibrate the user's historical preference in the recommended list while 0 indicates no calibration.  We can formalize the calibration optimization problem given the binary decision matrix, Z, as:

\begin{small}
\begin{equation}
\begin{aligned}
% \begin{small}
\max_{Z_{ui}} \quad & \sum_{u \in \mathcal{U}}\sum_{i=1}^{N}{S_{ui} \cdot Z_{ui}} - \lambda_1 \cdot \mathbf{MC}(Z^1,\mathcal{U})   \\
\textrm{s.t.} \quad & \sum_{i=1}^{N}{Z_{ui}} = K \quad,  \sum_{i=1}^{N}{Z^1_{ui}} = int(W(I_u) \cdot K) & \forall u \\ 
& Z^1_{ui} + Z^2_{ui} = Z_{ui} \quad,  Z^1_{ui}~, Z^2_{ui}~, Z_{ui} \in{\{0,1\}} & \forall u,i 
\end{aligned}
\label{eq:optimization}
\end{equation}
\end{small}

\noindent
where $Z^1_{ui}$ and $Z^2_{ui}$ are helper binary decision variables that indicate whether the item $Z_{ui}$ is selected due to improving miscalibration metric or a high predictive relevance score, respectively. The $int(.)$ function rounds the input to the nearest integer value. In our experiment, we define $W(I_u)$ based on the size of the user profile, formally as $W(I_u) = \min [\frac{|I_u|}{\frac{1}{\mathcal{|U|}}  \sum_{u\in \mathcal{U}}|I_u|}, 1]$ motivated by our analysis in Figure~\ref{fig:testvstrain_diff_ml_100K} and leave more rigorous definitions for future work. Additionally, as described in Section~\ref{sec:problem_definition}, MC represents the miscalibration metric by calculating the average divergence values for all users on a subset of the top-K list by size $int(W(I_u) \cdot K)$ denoted by $Z^1$ decision matrix. Given that the JS and H divergence functions are non-linear, for optimization purposes we adopt the \textit{Total Variation} function~\cite{chambolle2004algorithm,levin2017markov}  defined as the $\mathscr{l}_1$ norm between distributions of $p(c|u)$ and $q(c|u)$ to calculate divergence values. As a result of the linear objective function, the optimization problem becomes mixed-integer linear programming (MILP) that can be solved using heuristic algorithms (e.g., branch\&bound algorithms)  in industrial optimization solvers to provide a satisfactory solution in practice\footnote{In our experiment, we used the Gurobi solver at \url{https://www.gurobi.com}}. Note that our proposed model will obviously satisfy properties \textbf{P1} and \textbf{P2} when $\lambda_1 = 0$ as it will return the same baseline recommendation and will calibrate the recommendation list completely for all users when $W(I_u)= 1 ~\forall u$ and $\lambda_1$ is large. Varying weighting parameter $W(I_u)$ aims to satisfy the property \textbf{P3}.


==> bc/intro_bc.tex <==
\section{Introduction}
\label{sec:intro}
Recommender systems learn from user' behavior to infer their preference and recommend items to them that match their interests.
In doing so, various recommendation methods~\cite{abdollahpouri2019unfairness} would end up recommending  a small set of popular items, because they count for the majority of the user-item interaction and lead to higher accuracy metrics~\cite{abdollahpouri2020connection}. User profile calibration aims to address this problem by maintaining the categorical distribution of items in the recommendation list. 
For example, if a user profile consists of 9 comedy movies and 1 action movie, a calibrated recommender system would maintain the same 9:1 proportion of movie genres in its top-k recommendations. As a result, the recommendation list is more likely to include items from less popular item categories, cover a wider range of items, and be more diverse.

While the machine learning community has addressed calibration extensively~\cite{bella2010calibration}, it has gained attention in the recommendation community rather recently~\cite{steck2018calibrated,seymen2021constrained}. \citet{steck2018calibrated} proposes an iterative greedy algorithm to add the most relevant items to the recommendation list as long as they satisfy the calibration constraint. \citet{seymen2021constrained} argue that this approach is suboptimal because of the myopic nature of greedy algorithms, as well as the non-linearity of the Kullback–Leibler divergence used to measure calibration. They instead propose an optimization algorithm for calibration while maintaining model effectiveness.

Even though the research on calibrated recommendation aims to maintain a fair treatment for all the users, it mainly assumes that the algorithm's capacity for calibration is the same for all the users. For instance, user A with a profile size of 100 items is treated similarly to user B with a profile size of 10. We argue that the confidence in the categorical distribution of a user profile is proportional to their profile size. In this example, assume both users A and B have the 9:1 proportion of comedy vs.~action movies in the profiles. Figure~\ref{fig:beta_dist} shows the beta distribution\footnote{With a Bayesian view of the two user profiles, we Let $\theta_A$ and $\theta_B$ be the probability of user A and B watching a comedy movie during test time, respectively. Therefore, our posterior for $\theta_A$ would be $beta(91,11)$ and for $\theta_B$ would be $beta(10,2)$.} of both users watching a comedy movie in the test set ($\theta_A = beta(91,11)$ vs.~$\theta_B = beta(10,2)$). We see that user A is ~0.67 more likely to watch a comedy movie, indicating that the profile size has a critical factor in defining calibration confidence. The existing calibration methods, however, would treat the two profiles equally. We also show this property via empirical analysis in Figure~\ref{fig:testvstrain_diff_ml_100K} where we observe a higher miscalibration between test and train sets as the user profile size decreases (e.g., active vs.~inactive users).

In this work, we aim to address this issue by proposing a confidence-aware optimization-based re-ranking algorithm to find the balance between calibration and item diversity while maintaining different levels of confidence in modeling calibration for different users. Inspired by our theoretical analysis, we propose a weighting scheme to model calibration confidence for a given profile size. Our proposed optimization algorithm solves a multi-objective calibration problem where we also take into account the diverse and dynamic nature of user profiles. Our extensive experiments demonstrate the effectiveness of our proposed method, not only in terms of recommendation effectiveness but also in other beyond-accuracy metrics such as diversity. We further analyze the performance of our model for different user groups showing the effect of our weighting scheme for users of different profile sizes. Our contributions can be summarized as follows:

\begin{itemize}[leftmargin=*]
    \item Proposing a weighted mixed-integer linear programming model, called \ourmodel,  to solve our multi-objective calibration problem.
    \item Evaluating the proposed method against the state-of-the-art recommendation calibration method, applied on \textit{four} base recommendation algorithms and \textit{two} real-world datasets.
    \item Extensive empirical analysis of the results on various beyond-accuracy metrics such as diversity across \textit{three} user groups.\footnote{\url{https://github.com/rahmanidashti/CalibrationFair}}
\end{itemize}

==> sections/method.tex <==
\section{Proposed Method}
\label{sec:method}
\todo{@Ehsan}

\partitle{Formalizing the problem of calibration and its evaluation}
In this section, we outline metrics that quantify the degree of calibration of a list of recommended items, with respect to the user’s
profile. To this end, we consider two distributions,
both of which are based on the distribution of categories C for each
item  i, denoted by p(C|i), which is assumed to be given:
p(C|u): the distribution over genres C of the set of items $\mathcal{I}$
played by user u in the past:
q(C|u) : the distribution of genres C in the recommended list to user u

\partitle{Formalizing diversity and confidence definition}


\partitle{Proposing the optimization and algorithm to solve} 
In this section, we will use the top-N recommendation list and relevance scores provided by the traditional unfair recommendation algorithm as the baseline. We apply a re-ranking post-hoc algorithm to maximize the total sum of relevance scores while minimizing the deviation from the profile list in comparison to the recommended list, known as miscalibration, $\mathbf{MC}$. We can formulate the calibration optimization problem given the binary decision matrix, A, as:

\begin{small}
\begin{equation}
\begin{aligned}
% \begin{small}
\max_{A_{ui}} \quad & \sum_{u \in \mathcal{U}}\sum_{i=1}^{N}{S_{ui}.A_{ui}} - \lambda_1. \mathbf{MC}(A,\mathcal{U}) \\
\textrm{s.t.} \quad & \sum_{i=1}^{N}{A_{ui}} = K, A_{ui} \in{\{0,1\}}
% \end{small}
\end{aligned}
\label{eq:optimization}
\end{equation}
\end{small}

